Global BGP Attacks that Evade Route Monitoring

As the deployment of comprehensive Border Gateway Protocol (BGP) security measures is still in progress, BGP monitoring continues to play a critical role in protecting the Internet from routing attacks. Fundamentally, monitoring involves observing BGP feeds to detect suspicious announcements and taking defensive action. However, BGP monitoring relies on seeing the malicious BGP announcement in the first place! In this paper, we develop a novel attack that can hide itself from all state-of-the-art BGP monitoring systems we tested while affecting the entire Internet. The attack involves launching a sub-prefix hijack with the RFC-specified NO_EXPORT community attached to prevent networks with the malicious route installed from sending the route to BGP monitoring systems. We study the viability of this attack at four tier-1 networks and find all networks we studied were vulnerable to the attack. Finally, we propose a mitigation that significantly improves the robustness of the BGP monitoring ecosystem. Our paper aims to raise awareness of this issue and offer guidance to providers to protect against such attacks.

==> background.tex <==
\section{Background}
\subsection{Basic BGP Operation}
The Border Gateway Protocol (BGP) is used to exchange routes to groups of IP addresses (known as IP prefixes) between various Autonomous Systems (ASes) across the Internet. To route an IP prefix via BGP, an AS "originates" a BGP announcement containing the prefix it would like to have routed and sends this announcement to any neighboring ASes which it has a BGP session with (sometimes referred to as a BGP peering). These ASes process the BGP announcement and decide if it is their preferred route for reaching the prefix in question. If they prefer the new route over their previously used route (or if there was no previous route to that IP prefix), they install the new route and propagate the announcement further to other neighboring networks.

\subsection{Longest Prefix Match Routing and BGP}
In BGP announcements for different IP prefixes propagate independently. For each prefix heard in BGP, a router will compare different BGP announcements heard for that prefix and select the route it wants to use which is installed into its Routing Information Base (or RIB). When forwarding traffic, preference is always given for the most-specific prefix matching a given IP address.

\subsection{BGP Communities}
The core BGP routing protocol can be extended with BGP attributes that specify additional properties regarding a BGP message. One such attribute is the BGP communities attribute. BGP communities are unstructured 32-bit tags an AS can attach to a BGP route to convey additional properties of a BGP route~\cite{rfc1997_bgp_communities}. BGP communities are ``optionally transitive''~\cite{rfc1997_bgp_communities} meaning an AS can choose to pass BGP communities on to additional ASes or strip them off of a BGP announcement after processing. While some communities are strictly attached for informational purposes, others often referred to as action communities are used as signals to cause ASes to process BGP routes differently~\cite{birgelee2019sico}. The RFC which defined BGP communities introduced several ``well-known'' communities that ``shall be implemented in any community-attribute-aware BGP speaker''~\cite{RFC1997}. These communities include the NO\_EXPORT community which prohibits an AS from exporting a route beyond a confederation boundary~\cite{RFC1997}.

\subsection{BGP Attacks}
BGP was originally developed without authentication for the announcements made by various networks. This enables BGP attacks where an adversary makes malicious BGP announcements to redirect traffic for a variety of purposes~\cite{birge2018bamboozling, apostolaki2017bitcoin}. Generally BGP hijacks are divided into two types: equally-specific prefix hijacks and sub-prefix hijacks. In an equally-specific prefix hijack the adversary announces the same IP prefix as the victim network it is attacking, causing the adversary's and victim's announcement to compete with each other in the route-selection process. In a sub-prefix announcement the adversary announces uses longer sub-prefix in its announcement causing its announcement to spread uncontested through the Internet. When traffic is forwarded to the victim's network, longest-prefix-match forwarding causes ASes to use the adversary's route instead of the victim's

\subsection{BGP Monitoring}
While waiting for the deployment of robust BGP security improvements, BGP monitoring has come to plan an important role as a way of detecting BGP attacks~\cite{thousandeyes,ciscocrosswork,PHAS,DFOH,internetintel,codeBGP}.
These systems use BGP route monitors to collect BGP announcements heard from the Internet and feed them to various processing algorithms. These route monitors establish BGP peering with hundreds of networks~\cite{ris_peers, routeviews_peers} and record the announcements made to them by their peers. Peers that establish sessions with these monitoring services typically configure their routers to send all routes used to the monitoring service similar to if the monitoring service was one of their BGP customers (as BGP customers receive a full table of Internet routes). Using data from the various peers, BGP monitoring algorithms employ a variety of techniques to determine if a rout is suspicious. This includes checking the origin of announcements against databases of IP prefix ownership~\cite{phas_bgp_monitoring} and analyzing routes for various anomalies (e.g., large geographic gaps between consecutive ASes~\cite{dfoh}).

